Scaling up GANs for Text-to-Image Synthesis

The recent success of text-to-image synthesis has taken the world by storm and captured the general public's imagination. From a technical standpoint, it also marked a drastic change in the favored architecture to design generative image models. GANs used to be the de facto choice, with techniques like StyleGAN. With DALL-E 2, auto-regressive and diffusion models became the new standard for large-scale generative models overnight. This rapid shift raises a fundamental question: can we scale up GANs to benefit from large datasets like LAION? We find that na\"Ively increasing the capacity of the StyleGAN architecture quickly becomes unstable. We introduce GigaGAN, a new GAN architecture that far exceeds this limit, demonstrating GANs as a viable option for text-to-image synthesis. GigaGAN offers three major advantages. First, it is orders of magnitude faster at inference time, taking only 0.13 seconds to synthesize a 512px image. Second, it can synthesize high-resolution images, for example, 16-megapixel pixels in 3.66 seconds. Finally, GigaGAN supports various latent space editing applications such as latent interpolation, style mixing, and vector arithmetic operations.

==> Main_paper/Figures/Text2Img_model_sizes.tex <==
\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.7\linewidth]{Main_paper/Materials/figure_model_sizes.png}
    \vspace{-3mm}
    \caption{FID and CLIP curve of varying model sizes. (mock drawing)}
    \label{fig:model_size}
\end{figure}

==> Main_paper/Figures/Text2Img_training_curve.tex <==
\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.7\linewidth]{Main_paper/Materials/Training_curve.png}
    \vspace{-3mm}
    \caption{FID and CLIP curve as training progresses.}
    \label{fig:training_curve}
\end{figure}

==> Main_paper/Figures/character_variation.tex <==
\begin{figure}[b!]
    \centering
    \includegraphics[width=\figwidth]{Main_paper/Materials/fix_z_1col.pdf}
    \vspace{-4mm}
    \caption{ {\bf Role of the latent vector $\vb{z}$ and text embedding $\vb{t}$. } We generate images using $\vb{t}_i$ extracted from the prompt ``A cute baby monster character,", concatenated by the respective prompt for each column. Each row uses the same latent vector $\vb{z}_i$, which yields a similar composition and attributes.}
    \label{fig:character_variation}
\end{figure}

==> Main_paper/Figures/superres_horse_cropped.tex <==
\begin{figure*}[!ht]
    \centering
    \includegraphics[width=\figwidth]{Main_paper/Materials/superres_horse_cropped.pdf}
    \vspace{-0mm}
    \caption{\tae{{\bf Our GAN-based upsampler} is better and faster than baselines. This is a real input image but can be useful for ai generated image. The 4K horse image is cropped for full page layout. Any suggestions on the layout is welcome!}}
    \vspace{-4mm}
    \label{fig:superres_horse_taller}
\end{figure*}

==> Main_paper/Figures/superres_horse_taller.tex <==
\begin{figure*}[!ht]
    \centering
    \includegraphics[width=\figwidth]{Main_paper/Materials/superres_horse_taller.pdf}
    \vspace{-0mm}
    \caption{\tae{{\bf Our GAN-based upsampler} is better and faster than baselines. This is a real input image but can be useful for ai generated image. }}
    \vspace{-4mm}
    \label{fig:superres_horse_taller}
\end{figure*}

==> Main_paper/Figures/superres_horse_wider.tex <==
\begin{figure*}[!ht]
    \centering
    \includegraphics[width=\figwidth]{Main_paper/Materials/superres_horse_wider.pdf}
    \vspace{-4mm}
    \caption{\tae{{\bf Our GAN-based upsampler} is better and faster than baselines. This is a real input image but can be useful for ai generated image. }}
    \vspace{-4mm}
    \label{fig:superres_horse_wider}
\end{figure*}

==> Main_paper/Tables/Ablation.tex <==
\begin{table}[t]
\caption{\textbf{Ablation study on 64px text-to-image synthesis.} To evaluate the effectiveness of our components, we start with a modified version of StyleGAN for text conditioning. While increasing the network width does not show satisfactory improvement, each addition of our contributions keeps improving metrics. Finally, we increase the network width, and the model still responds well to scaling. All models are trained for 100k iterations at batch size of 256. }
\vspace{-2mm}
\resizebox{0.49\textwidth}{!}{
\begin{tabular}{lccc}
\cmidrule[1.0pt]{1-4}
Model                     & Zero-shot FID-10k & CLIP Score & Model size\\
\cmidrule[1.0pt]{1-4}
StyleGAN2 backbone~\cite{karras2020analyzing} &  29.91 & 0.222 & 27.8M \\
~~~~~~+~Larger (4.4$\times$)  & 27.41 & 0.226 & 123.0M \\
\cmidrule[0.5pt]{1-4}
~~+~Tuned & 28.11 & 0.228 &  26.2M \\
~~+~Attention      &  23.87  & 0.235 & 59.0M \\
~~+~Mixing augmentation & 21.66 &  0.254 & 59.0M\\
~~+~Adaptive convolution  & 19.97 & 0.261 & 80.2M\\
~~+~Deeper         & 19.03 & 0.264 & 135.3M \\
~~~~~~+~Larger (1.3$\times$) & 16.71 & 0.269 &  170.0M \\
~~+~Vision-aided GAN~\cite{kumari2021ensembling} & 15.43 & 0.272 & 135.3M \\
\cmidrule[1.0pt]{1-4}
\end{tabular}
}
\label{tab:ablation}
\end{table}

==> Main_paper/Tables/ImageNet64.tex <==
\begin{table}[t]
\caption{Class-conditional image generation results on ImageNet 64$\times$64.}
\vspace{-1mm}
\resizebox{0.4675\textwidth}{!}{
\begin{tabular}{lcccc}
\cmidrule[1.0pt]{1-5}
 Model & IS & FID & Precision & Recall \\
\cmidrule[1.0pt]{1-5}
BigGAN-Deep & - & 4.06 & 0.79 & 0.48 \\
ADM-G       & - & 2.07 & 0.74 & 0.63 \\
StyleGAN-XL & - & 1.51 & - & - \\
CDM         & 67.95 & 1.48 & - & - \\
\cmidrule[1.0pt]{1-5}
Ours + G       &    & 2.11 &           & \\
Ours + CLIP + G &    & 1.71 &           & \\
\cmidrule[1.0pt]{1-5}
\end{tabular}}
\label{table:imagenet64}
\end{table}

==> Main_paper/Tables/Text2Img256.tex <==
\begin{table}[t]

\caption{ { \bf Comparison on 256px text-to-image generation} using COCO zero-shot FID with 30k samples. LDM~\cite{rombach2022high}, Stable Diffusion~\cite{stablediffusion}, and Parti~\cite{yu2022scaling} provide models of comparable size to ours. [Base] and [Upsampler] indicate model size of each component. [Steps] indicates the number of forward passes of the model at inference. [MAC] measures the multiply-accumulate op count.}
\vspace{-1mm}
\resizebox{0.495\textwidth}{!}{
\begin{tabular}{lccccc}
\cmidrule[1.0pt]{1-6}

Model    & Base & Upsampler & Steps & MACs(T) & Zero-shot FID  \\
\cmidrule[1.0pt]{1-6}
LDM-KL-8~\cite{rombach2022high}   & 1.45B & - & 250 & - &23.31   \\
LDM-KL-8-G~\cite{rombach2022high} & 1.45B & - & 500 & - &12.63   \\
Stable Diffusion~\cite{stablediffusion}  & 860M & - & 500 & 171.0 & 14.96  \\
Parti 750M~\cite{yu2022scaling} & 750M & - & 1024 & - & 10.71 \\
\cmidrule[0.5pt]{1-6}
DALL$\cdot$E 2~\cite{ramesh2022hierarchical}  & 4.5B & 700M & 527 & - & 10.39 \\
Imagen~\cite{saharia2022photorealistic}  & 2.0B & 600M & - & - & 7.27  \\

Parti 20B~\cite{yu2022scaling}  & 20B & - & 1024 & - & 7.23  \\
\cmidrule[1.0pt]{1-6}
Ours     & 370M  & 390M & 1 & 0.255 & 15.29 \\
\cmidrule[1.0pt]{1-6}
\label{tab:t2i256}
\end{tabular}}
\vspace{-5.5mm}
\end{table}

==> Main_paper/Tables/Text2Img64.tex <==
\begin{table}[t]
\caption{ {\bf Comparison with Imagen on 64px text-to-image synthesis.} The FID~\cite{Heusel2017GANsTB} and CLIP score~\cite{hessel2021clipscore} of Imagen are taken from the measurements used to create Figure 4(b) of the Imagen paper. $^*$Imagen measures CLIP score using a proprietary CLIP model with the same architecture. Imagen-G indicates Imagen with classifier-free guidance.}
\vspace{-2mm}
\resizebox{0.47\textwidth}{!}{
\begin{tabular}{lccc}
\cmidrule[1.0pt]{1-4}
Model    & Zero-shot FID-10k & CLIP score & Model size\\
\cmidrule[1.0pt]{1-4}
Imagen (small)~\cite{saharia2022photorealistic}   & 11.35 & 0.245$^{*}$ & 300M\\
Imagen-G (small)~\cite{saharia2022photorealistic} & 9.40 & 0.265$^{*}$ & 300M\\
\cmidrule[1.0pt]{1-4}
Ours     & 9.92 & 0.282 & 370M\\
~~+Vision-aided GAN~\cite{kumari2021ensembling}     & 9.35 & 0.288 & 370M\\
\cmidrule[1.0pt]{1-4}
\end{tabular}}
\label{table:t2i64}
\vspace{-2mm}
\end{table}
